Non-Primordial Contribution to the Cosmic Microwave Background

The cosmic microwave background is interpreted as relic thermal radiation from the epoch of recombination at z~1090. Recent work by Gjergo & Kroupa (GK25) have challenged this assumption proposing that dust-enshrouded starbursts in the progenitors of massive early-type galaxies at z~15-20 contribute to the CMB at the percent level of the present-day CMB energy density. Existing test of this scenario rely on CMB monopole; here we present the first test against the CMB anisotropy power spectrum, which probes the dynamical imprint of the radiation content on the sound horizon and acoustic peaks. We introduce a single parameter $\varepsilon_{\rm CMB}$ that rescales the primordial photon energy density above a redshift (z=17). Constraining the model with the Planck 2018, lensing likelihoods and BAO measurements, we find a percent-level dust contribution to be fully consistent with the data. When we restrict $\varepsilon_{\rm CMB}\leq1$, the data place a 68 (95) per cent lower bound $\varepsilon_{\rm CMB}\gtrsim 0.971$(0.953), permitting a non-primordial contribution of up to ~3 (~5) per cent of the CMB energy density. When sampled with $\varepsilon_{\rm CMB}$ as a free parameter, the data yield a well-resolved posterior with $\varepsilon_{\rm CMB} = 1.0104^{+0.025}_{-0.024}$. The 1.4 per cent contribution conservatively estimated by GK25 lies within the 1$\sigma$ region of both cases, whereas a contribution approaching the full CMB energy density is excluded at 42$\sigma$. Treating z as a free parameter returns a flat posterior across 5<z<50 indicating the anisotropy constrains the dust contribution, but not when it occurs. The standard LCDM parameters are recovered without significant shifts, showing that current CMB precision cosmology has sufficient room to accommodate a dust contribution at the level predicted by GK25 without detectable consequence for parameter inference.

==> abstract.tex <==
The cosmic microwave background is interpreted as relic thermal radiation from the epoch of recombination at z~1090. Recent work by Gjergo & Kroupa (GK25) have challenged this assumption proposing that dust-enshrouded starbursts in the progenitors of massive early-type galaxies at z~15-20 contribute to the CMB at the percent level of the present-day CMB energy density. Existing test of this scenario rely on CMB monopole; here we present the first test against the CMB anisotropy power spectrum, which probes the dynamical imprint of the radiation content on the sound horizon and acoustic peaks. We introduce a single parameter $\varepsilon_{\rm CMB}$ that rescales the primordial photon energy density above a redshift (z=17). Constraining the model with the Planck 2018, lensing likelihoods and BAO measurements, we find a percent-level dust contribution to be fully consistent with the data. When we restrict $\varepsilon_{\rm CMB}\leq1$, the data place a 68 (95) per cent lower bound $\varepsilon_{\rm CMB}\gtrsim 0.971$(0.953), permitting a non-primordial contribution of up to ~3 (~5) per cent of the CMB energy density. When sampled with $\varepsilon_{\rm CMB}$ as a free parameter, the data yield a well-resolved posterior with $\varepsilon_{\rm CMB} = 1.0104^{+0.025}_{-0.024}$. The 1.4 per cent contribution conservatively estimated by GK25 lies within the 1$\sigma$ region of both cases, whereas a contribution approaching the full CMB energy density is excluded at 42$\sigma$. Treating z as a free parameter returns a flat posterior across 5<z<50 indicating the anisotropy constrains the dust contribution, but not when it occurs. The standard LCDM parameters are recovered without significant shifts, showing that current CMB precision cosmology has sufficient room to accommodate a dust contribution at the level predicted by GK25 without detectable consequence for parameter inference.
